A Brief Introduction to Causal Inference in Machine Learning

This is a lecture note produced for DS-GA 3001.003 "Special Topics in DS - Causal Inference in Machine Learning" at the Center for Data Science, New York University in Spring, 2024. This course was created to target master's and PhD level students with basic background in machine learning but who were not exposed to causal inference or causal reasoning in general previously. In particular, this course focuses on introducing such students to expand their view and knowledge of machine learning to incorporate causal reasoning, as this aspect is at the core of so-called out-of-distribution generalization (or lack thereof.)

==> math_preamble.tex <==
% IMPORTS

% MATH SHORTHANDS
% Partial Differential of #1 w.r.t. #2
\newcommand{\dpartial}[2]{\frac{\partial #1}{\partial #2}}

% \ceil{x} instead of \lceil x \rceil
% Same for \floor{x}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\abs}[1]{\left| #1 \right|}

% Auto-resize () and []
\newcommand*\autoop{\left(}
\newcommand*\autocp{\right)}
\newcommand*\autoob{\left[}
\newcommand*\autocb{\right]}
\AtBeginDocument {%
   \mathcode`( 32768
   \mathcode`) 32768
   \mathcode`[ 32768
   \mathcode`] 32768
   \begingroup
       \lccode`\~`(
       \lowercase{%
   \endgroup
       \let~\autoop
   }\begingroup
       \lccode`\~`)
       \lowercase{%
   \endgroup
       \let~\autocp
   }\begingroup
       \lccode`\~`[
       \lowercase{%
   \endgroup
       \let~\autoob
   }\begingroup
       \lccode`\~`]
       \lowercase{%
   \endgroup
       \let~\autocb
}}
\delimiterfactor 1001
\makeatletter
\AtBeginDocument {%
          \def\resetMathstrut@{%
           \setbox\z@\hbox{\the\textfont\symoperators\char40}%
           \ht\Mathstrutbox@\ht\z@ \dp\Mathstrutbox@\dp\z@}%
}%
\makeatother

\newcommand{\vecbr}[1]{\langle #1 \rangle}

% Unit vectors

\newcommand{\ui}{\hat{\imath}}
\newcommand{\uj}{\hat{\jmath}}
\newcommand{\uk}{\hat{k}}
\newcommand{\V}{\vec{V}}

% Common expressions

\newcommand{\half}[1]{\frac{#1}{2}}
\newcommand{\recip}[1]{\frac{1}{#1}}
\newcommand{\invsqrt}[1]{\recip{\sqrt{#1}}}
\newcommand{\halfpi}{\half{\pi}}

% Integral evaluation bar
\newcommand{\windbar}[2]{\Big|_{#1}^{#2}}
\newcommand{\rightinfwindbar}[0]{\Big|_{0}^\infty}
\newcommand{\leftinfwindbar}[0]{\Big|_{-\infty}^0}

% Column type "L" for tabular environment, contents of column are in display mode by default
\newcolumntype{L}{>{$}l<{$}}

% Circled single character (used for state machine notation)

\newcommand{\state}[1]{\large\protect\textcircled{\textbf{\small#1}}}

% FORMATTING
% Remove section numbers
\makeatletter
\renewcommand{\@seccntformat}[1]{}
\makeatother
% Indent text within section
% \leftskip=2em
% Center section headings
\titleformat{\section}[block]{\Large\bfseries\filcenter}{}{1em}{}
% `enumerate` environment uses (\alph) format
\setlist[enumerate]{label=(\alph*)}

\newcommand{\shrule}{\\ \centerline{\rule{13cm}{0.4pt}}}

% QUANTUM 

\usepackage{mathtools}
\DeclarePairedDelimiter\bra{\langle}{\rvert}
\DeclarePairedDelimiter\ket{\lvert}{\rangle}
\DeclarePairedDelimiterX\braket[2]{\langle}{\rangle}{#1 \delimsize\vert #2}
\DeclarePairedDelimiterX\brakaket[3]{\langle}{\rangle}{#1 \delimsize\vert #2 \delimsize\vert #3}
\newcommand{\tbra}[1]{$\bra{#1}$}
\newcommand{\tket}[1]{$\ket{#1}$}
\newcommand{\tbraket}[2]{$\braket{1}{2}$}
\newcommand{\infint}[0]{\int_{-\infty}^{\infty}}
\newcommand{\rightinfint}[0]{\int_0^\infty}
\newcommand{\leftinfint}[0]{\int_{-\infty}^0}
\newcommand{\wavefuncint}[1]{\infint|#1|^2}
\newcommand{\ham}[0]{\hat{H}}
